LV-Eval: A Balanced Long-Context Benchmark with 5 Length Levels Up to 256K

State-of-the-art large language models (LLMs) are now claiming remarkable supported context lengths of 256k or even more. In contrast, the average context lengths of mainstream benchmarks are insufficient (5k-21k), and they suffer from potential knowledge leakage and inaccurate metrics, resulting in biased evaluation. This paper introduces LV-Eval, a challenging long-context benchmark with five length levels (16k, 32k, 64k, 128k, and 256k) reaching up to 256k words. LV-Eval features two main tasks, single-hop QA and multi-hop QA, comprising 11 bilingual datasets. The design of LV-Eval has incorporated three key techniques, namely confusing facts insertion, keyword and phrase replacement, and keyword-recall-based metric design. The advantages of LV-Eval include controllable evaluation across different context lengths, challenging test instances with confusing facts, mitigated knowledge leakage, and more objective evaluations. We evaluate 15 LLMs on LV-Eval and conduct ablation studies on the benchmarking techniques. The results reveal that: (i) Moonshot-v1 and recent large-scale open-source models, such as Qwen-2.5-72B and Llama-3.1-70B, achieve the highest performance on LV-Eval, particularly at lengths below 64k. (ii) Models exhibit distinct score trends. For example, GLM-4-9B-128k, Yi-6B-200k, and Llama3-8B-1M exhibit a relatively gentle degradation of performance, but their absolute performances may not necessarily be higher than those of LLMs with shorter context lengths. (iii) LLMs' performances can significantly degrade in the presence of confusing information, especially in the pressure test of "needle in a haystack". (iv) Issues related to knowledge leakage and inaccurate metrics introduce bias in evaluation, and these concerns are alleviated in LV-Eval. All datasets and evaluation codes are released at: https://github.com/infinigence/LVEval.

==> Tables/res_ablt_study_ci_kpr.tex <==
% \begin{table}[t]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}lllllllllllllllll@{}}
% \toprule
% model                              & ablation             & \multicolumn{5}{c}{hotpotwikiqa\_mixup} & \multicolumn{5}{c}{multifieldqa\_en\_mixup} & \multicolumn{5}{c}{multifieldqa\_zh\_mixup} \\ \midrule
% \multirow{4}{*}{Ll.4}      & both                     & 3.91   & 1.87   & 1.15  & 0.74  & 0.88  & 8.64    & 5.14    & 1.93   & 2.19   & 1.02  & 4.66    & 1.26    & 1.04   & 0.21   & 0.57  \\
%                                          & replace     & 4.1    & 1.56   & 1.36  & 0.63  & 0.88  & 8.43    & 4.84    & 1.93   & 2.46   & 0.95  & 5.45    & 1.26    & 1.06   & 0.21   & 0.57  \\
%                                          & insert & 6.29   & 2.47   & 3.37  & 1.47  & 1.57  & 9.05    & 6.08    & 3.29   & 3.59   & 1.44  & 4.83    & 2.06    & 0.71   & 0.3    & 0.42  \\
%                                          & baseline              & 6.48   & 2.48   & 2.98  & 1.29  & 1.57  & 9.65    & 6.08    & 3.29   & 3.59   & 1.67  & 5.49    & 2.17    & 0.62   & 0.3    & 0.42  \\ \cmidrule(l){1-17}
% \multirow{4}{*}{ch.}         & both                     & 18.2  & 13.8  & 10.6 & 8.4   & 6.71  & 25.88   & 13.21   & 10.49  & 8.94   & 4.46  & 31.22   & 23.99   & 21.54  & 10.47  & 7.42  \\
%                                          & replace     & 21.32  & 13.04  & 9.99  & 6.56  & 6.12  & 33.54   & 17.27   & 12.15  & 8.94   & 4.44  & 44.9    & 40.23   & 23.03  & 14.26  & 7.5   \\
%                                          & insert & 27.06  & 24.75  & 17.57 & 12.89 & 10.88 & 31.97   & 19.8    & 14.12  & 10.54  & 6.4   & 33.24   & 28.38   & 20.75  & 15.84  & 8.96  \\
%                                          & baseline              & 28.48  & 21.96  & 18.89 & 11.31 & 10.69 & 41.46   & 24.29   & 14.32  & 10.31  & 6.24  & 44.8    & 42.65   & 27.66  & 17.73  & 9.51  \\ \cmidrule(l){1-17}
% \multirow{4}{*}{lo.}    & both                     & 11.7   & 9.31   & 4.22  & 5.49  & 3.01  & 11.66   & 8.03    & 5.75   & 3.09   & 4.68  & 9.9     & 9.03    & 4.44   & 3.44   & 3.92  \\
%                                          & replace     & 11.07  & 6.17   & 5.27  & 5.31  & 3.06  & 15.32   & 10.61   & 6.49   & 3.02   & 4.94  & 11.29   & 10.24   & 4.24   & 3.6    & 3.89  \\
%                                          & insert & 19.48  & 14.33  & 9.41  & 11.34 & 6.44  & 15.56   & 8.77    & 13.16  & 9.88   & 8.65  & 13.5    & 9.76    & 4.27   & 4      & 3.82  \\
%                                          & baseline              & 18.79  & 12.44  & 9.94  & 11.33 & 7.47  & 20.45   & 12.91   & 11.69  & 9.28   & 8.59  & 16.59   & 11.31   & 5.13   & 3.96   & 3.82  \\ \cmidrule(l){1-17}
% \multirow{4}{*}{Ll.32} & both                     & 3.73   & 2.43   & 2.25  & 2.03  & 1.63  & 7.92    & 5.56    & 3.78   & 3.9    & 3.09  & 4.84    & 4.13    & 1.42   & 2.38   & 1.17  \\
%                                          & replace     & 4.41   & 2.67   & 2.37  & 2.04  & 1.39  & 11.09   & 6.2     & 3.06   & 3.62   & 3.45  & 5.99    & 3.88    & 1.92   & 2.72   & 1.17  \\
%                                          & insert & 5.13   & 3.23   & 4.77  & 3.53  & 2.81  & 7.81    & 6.12    & 3.92   & 4.03   & 3.38  & 4.12    & 5.1     & 2.13   & 1.64   & 2.29  \\
%                                          & baseline              & 5.44   & 3.98   & 4.85  & 3.28  & 2.78  & 11.86   & 6.84    & 4.75   & 3.95   & 3.34  & 7.62    & 5.04    & 2.37   & 1.73   & 2.29  \\ \cmidrule(l){1-17}
% \multirow{4}{*}{yi.}              & both                     & 20.12  & 14.8   & 9.07  & 5.82  & 4     & 10.21   & 9.72    & 9.17   & 6.03   & 5.63  & 2.99    & 1.47    & 2.47   & 2.78   & 1.24  \\
%                                          & replace     & 23.84  & 13.77  & 6.52  & 6.69  & 3.84  & 12.69   & 13.67   & 11.05  & 7.3    & 5.7   & 4.62    & 4.43    & 2.51   & 3.6    & 2.18  \\
%                                          & insert & 33.32  & 16.89  & 11    & 7.62  & 8.09  & 12.02   & 9.7     & 11.19  & 5.91   & 7.29  & 3.32    & 2.69    & 2.67   & 2.95   & 1.8   \\
%                                          & baseline              & 30.71  & 17.62  & 10.43 & 10.17 & 8.51  & 16.78   & 13.35   & 12.38  & 7.83   & 7.27  & 4.47    & 5.61    & 3.58   & 4.07   & 2.59  \\ \cmidrule(l){1-17}
% \multirow{4}{*}{vi.}      & both                     & 2.83   & 1.87   & 1.18  & 1.24  & 1.98  & 8.32    & 4.14    & 3.05   & 2.65   & 1.74  & 5.68    & 4.7     & 1.97   & 0.87   & 1.12  \\
%                                          & replace     & 2.09   & 1.63   & 1.27  & 1.13  & 1.98  & 8.07    & 4.32    & 2.67   & 2.65   & 1.31  & 8.18    & 4.7     & 1.81   & 0.89   & 0.96  \\
%                                          & insert & 5.84   & 3.58   & 2.6   & 1.82  & 1.09  & 9.02    & 6.66    & 5.4    & 2.94   & 2.37  & 10.03   & 5.7     & 2.62   & 3.42   & 1.99  \\
%                                          & baseline              & 5.81   & 4.09   & 3.3   & 1.48  & 1.22  & 9.49    & 6.88    & 5.52   & 2.9    & 2.09  & 10.22   & 5.77    & 3.08   & 3      & 1.83  \\ \cmidrule(l){1-17} 
% \end{tabular}
% }
% \caption{\label{tab:res_ablt_study_ci_kpr}Results of ablation study on confusing facts insertion and keyword and phrase replacement. The abbreviations for ch., yi., lo., Ll.32, vi., and Ll.4 represent for Chatglm3-6B-32k, Yi-6B-200k, Longchat-7B-v1.5-32k, Llama-2-7B-32k-Instruct, Vicuna-7B-v1.5-16k, and Llama2-7B-chat-4k, respectively.}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{model} &
  \multirow{2}{*}{ablation} &
  \multicolumn{5}{c}{hotpotwikiqa\_mixup} &
  \multicolumn{5}{c}{multifieldqa\_en\_mixup} &
  \multicolumn{5}{c}{multifieldqa\_zh\_mixup} \\ \cline{3-17} 
 &
   &
  $16k$ &
  $32k$ &
  $64k$ &
  $128k$ &
  $256k$ &
  $16k$ &
  $32k$ &
  $64k$ &
  $128k$ &
  $256k$ &
  $16k$ &
  $32k$ &
  $64k$ &
  $128k$ &
  $256k$ \\ \hline
Ll.4 &
  \multicolumn{1}{l|}{both} &
  3.91 &
  1.87 &
  1.15 &
  0.74 &
  \multicolumn{1}{l|}{0.88} &
  8.64 &
  5.14 &
  1.93 &
  2.19 &
  \multicolumn{1}{l|}{1.02} &
  4.66 &
  1.26 &
  1.04 &
  0.21 &
  0.57 \\
 &
  \multicolumn{1}{l|}{replace} &
  4.1 &
  1.56 &
  1.36 &
  0.63 &
  \multicolumn{1}{l|}{0.88} &
  8.43 &
  4.84 &
  1.93 &
  2.46 &
  \multicolumn{1}{l|}{0.95} &
  5.45 &
  1.26 &
  1.06 &
  0.21 &
  0.57 \\
 &
  \multicolumn{1}{l|}{insert} &
  6.29 &
  2.47 &
  3.37 &
  1.47 &
  \multicolumn{1}{l|}{1.57} &
  9.05 &
  6.08 &
  3.29 &
  3.59 &
  \multicolumn{1}{l|}{1.44} &
  4.83 &
  2.06 &
  0.71 &
  0.3 &
  0.42 \\
 &
  \multicolumn{1}{l|}{baseline} &
  6.48 &
  2.48 &
  2.98 &
  1.29 &
  \multicolumn{1}{l|}{1.57} &
  9.65 &
  6.08 &
  3.29 &
  3.59 &
  \multicolumn{1}{l|}{1.67} &
  5.49 &
  2.17 &
  0.62 &
  0.3 &
  0.42 \\ \hline
\multirow{4}{*}{ch.} &
  \multicolumn{1}{l|}{both} &
  18.2 &
  13.8 &
  10.6 &
  8.4 &
  \multicolumn{1}{l|}{6.71} &
  25.88 &
  13.21 &
  10.49 &
  8.94 &
  \multicolumn{1}{l|}{4.46} &
  31.22 &
  23.99 &
  21.54 &
  10.47 &
  7.42 \\
 &
  \multicolumn{1}{l|}{replace} &
  21.32 &
  13.04 &
  9.99 &
  6.56 &
  \multicolumn{1}{l|}{6.12} &
  33.54 &
  17.27 &
  12.15 &
  8.94 &
  \multicolumn{1}{l|}{4.44} &
  44.9 &
  40.23 &
  23.03 &
  14.26 &
  7.5 \\
 &
  \multicolumn{1}{l|}{insert} &
  27.06 &
  24.75 &
  17.57 &
  12.89 &
  \multicolumn{1}{l|}{10.88} &
  31.97 &
  19.8 &
  14.12 &
  10.54 &
  \multicolumn{1}{l|}{6.4} &
  33.24 &
  28.38 &
  20.75 &
  15.84 &
  8.96 \\
 &
  \multicolumn{1}{l|}{baseline} &
  28.48 &
  21.96 &
  18.89 &
  11.31 &
  \multicolumn{1}{l|}{10.69} &
  41.46 &
  24.29 &
  14.32 &
  10.31 &
  \multicolumn{1}{l|}{6.24} &
  44.8 &
  42.65 &
  27.66 &
  17.73 &
  9.51 \\ \hline
\multirow{4}{*}{lo.} &
  \multicolumn{1}{l|}{both} &
  11.7 &
  9.31 &
  4.22 &
  5.49 &
  \multicolumn{1}{l|}{3.01} &
  11.66 &
  8.03 &
  5.75 &
  3.09 &
  \multicolumn{1}{l|}{4.68} &
  9.9 &
  9.03 &
  4.44 &
  3.44 &
  3.92 \\
 &
  \multicolumn{1}{l|}{replace} &
  11.07 &
  6.17 &
  5.27 &
  5.31 &
  \multicolumn{1}{l|}{3.06} &
  15.32 &
  10.61 &
  6.49 &
  3.02 &
  \multicolumn{1}{l|}{4.94} &
  11.29 &
  10.24 &
  4.24 &
  3.6 &
  3.89 \\
 &
  \multicolumn{1}{l|}{insert} &
  19.48 &
  14.33 &
  9.41 &
  11.34 &
  \multicolumn{1}{l|}{6.44} &
  15.56 &
  8.77 &
  13.16 &
  9.88 &
  \multicolumn{1}{l|}{8.65} &
  13.5 &
  9.76 &
  4.27 &
  4 &
  3.82 \\
 &
  \multicolumn{1}{l|}{baseline} &
  18.79 &
  12.44 &
  9.94 &
  11.33 &
  \multicolumn{1}{l|}{7.47} &
  20.45 &
  12.91 &
  11.69 &
  9.28 &
  \multicolumn{1}{l|}{8.59} &
  16.59 &
  11.31 &
  5.13 &
  3.96 &
  3.82 \\ \hline
\multirow{4}{*}{Ll.32} &
  \multicolumn{1}{l|}{both} &
  3.73 &
  2.43 &
  2.25 &
  2.03 &
  \multicolumn{1}{l|}{1.63} &
  7.92 &
  5.56 &
  3.78 &
  3.9 &
  \multicolumn{1}{l|}{3.09} &
  4.84 &
  4.13 &
  1.42 &
  2.38 &
  1.17 \\
 &
  \multicolumn{1}{l|}{replace} &
  4.41 &
  2.67 &
  2.37 &
  2.04 &
  \multicolumn{1}{l|}{1.39} &
  11.09 &
  6.2 &
  3.06 &
  3.62 &
  \multicolumn{1}{l|}{3.45} &
  5.99 &
  3.88 &
  1.92 &
  2.72 &
  1.17 \\
 &
  \multicolumn{1}{l|}{insert} &
  5.13 &
  3.23 &
  4.77 &
  3.53 &
  \multicolumn{1}{l|}{2.81} &
  7.81 &
  6.12 &
  3.92 &
  4.03 &
  \multicolumn{1}{l|}{3.38} &
  4.12 &
  5.1 &
  2.13 &
  1.64 &
  2.29 \\
 &
  \multicolumn{1}{l|}{baseline} &
  5.44 &
  3.98 &
  4.85 &
  3.28 &
  \multicolumn{1}{l|}{2.78} &
  11.86 &
  6.84 &
  4.75 &
  3.95 &
  \multicolumn{1}{l|}{3.34} &
  7.62 &
  5.04 &
  2.37 &
  1.73 &
  2.29 \\ \hline
\multirow{4}{*}{yi.} &
  \multicolumn{1}{l|}{both} &
  20.12 &
  14.8 &
  9.07 &
  5.82 &
  \multicolumn{1}{l|}{4} &
  10.21 &
  9.72 &
  9.17 &
  6.03 &
  \multicolumn{1}{l|}{5.63} &
  2.99 &
  1.47 &
  2.47 &
  2.78 &
  1.24 \\
 &
  \multicolumn{1}{l|}{replace} &
  23.84 &
  13.77 &
  6.52 &
  6.69 &
  \multicolumn{1}{l|}{3.84} &
  12.69 &
  13.67 &
  11.05 &
  7.3 &
  \multicolumn{1}{l|}{5.7} &
  4.62 &
  4.43 &
  2.51 &
  3.6 &
  2.18 \\
 &
  \multicolumn{1}{l|}{insert} &
  33.32 &
  16.89 &
  11 &
  7.62 &
  \multicolumn{1}{l|}{8.09} &
  12.02 &
  9.7 &
  11.19 &
  5.91 &
  \multicolumn{1}{l|}{7.29} &
  3.32 &
  2.69 &
  2.67 &
  2.95 &
  1.8 \\
 &
  \multicolumn{1}{l|}{baseline} &
  30.71 &
  17.62 &
  10.43 &
  10.17 &
  \multicolumn{1}{l|}{8.51} &
  16.78 &
  13.35 &
  12.38 &
  7.83 &
  \multicolumn{1}{l|}{7.27} &
  4.47 &
  5.61 &
  3.58 &
  4.07 &
  2.59 \\ \hline
\multirow{4}{*}{vi.} &
  \multicolumn{1}{l|}{both} &
  2.83 &
  1.87 &
  1.18 &
  1.24 &
  \multicolumn{1}{l|}{1.98} &
  8.32 &
  4.14 &
  3.05 &
  2.65 &
  \multicolumn{1}{l|}{1.74} &
  5.68 &
  4.7 &
  1.97 &
  0.87 &
  1.12 \\
 &
  \multicolumn{1}{l|}{replace} &
  2.09 &
  1.63 &
  1.27 &
  1.13 &
  \multicolumn{1}{l|}{1.98} &
  8.07 &
  4.32 &
  2.67 &
  2.65 &
  \multicolumn{1}{l|}{1.31} &
  8.18 &
  4.7 &
  1.81 &
  0.89 &
  0.96 \\
 &
  \multicolumn{1}{l|}{insert} &
  5.84 &
  3.58 &
  2.6 &
  1.82 &
  \multicolumn{1}{l|}{1.09} &
  9.02 &
  6.66 &
  5.4 &
  2.94 &
  \multicolumn{1}{l|}{2.37} &
  10.03 &
  5.7 &
  2.62 &
  3.42 &
  1.99 \\
 &
  \multicolumn{1}{l|}{baseline} &
  5.81 &
  4.09 &
  3.3 &
  1.48 &
  \multicolumn{1}{l|}{1.22} &
  9.49 &
  6.88 &
  5.52 &
  2.9 &
  \multicolumn{1}{l|}{2.09} &
  10.22 &
  5.77 &
  3.08 &
  3 &
  1.83 \\ \hline
\end{tabular}%
}
\caption{Ablation results for confusing facts insertion (CFI) and keyword and phrase replacement (KPR). The abbreviations ``ch.'', ``yi.'', ``lo.'', ``Ll.32'', ``vi.'', and ``Ll.4'' stand for ChatGLM3-6B-32k, Yi-6B-200k, LongChat-7B-32k-v1.5, Llama2-7B-32k-Instruct, Vicuna-7B-16k-v1.5, and Llama2-7B-Chat-hf, respectively.}
\label{tab:res_ablt_study_ci_kpr}
\end{table}

==> Tables/res_factrecall.tex <==
% \begin{table}[t]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}cccccccccccc@{}}
% \toprule
% model                              & ablation             & \multicolumn{5}{c}{factrecall\_en}    & \multicolumn{5}{c}{factrecall\_zh}    \\ \midrule
% \multirow{4}{*}{Ll.4}      & both                     & 1.46  & 0.77  & 0.54  & 0.23  & 0.08  & 0     & 0     & 0     & 0     & 0     \\
%                                          & replace     & 1.62  & 0.77  & 0.54  & 0.23  & 0.08  & 0     & 0     & 0     & 0     & 0     \\
%                                          & insert & 3.47  & 2.12  & 2.06  & 2.15  & 2.38  & 0     & 0     & 0     & 0     & 0     \\
%                                          & baseline              & 4.01  & 3.06  & 2.78  & 2.62  & 2.57  & 1.07  & 0.92  & 0.8   & 0.71  & 0.64  \\ \cmidrule(l){1-12}
% \multirow{4}{*}{ch.}         & both                     & 95.5  & 82    & 44    & 22.25 & 11    & 0     & 2     & 12.5  & 9     & 7     \\
%                                          & replace     & 100   & 92.5  & 46.5  & 23.5  & 11.5  & 91.83 & 78    & 41    & 17.17 & 8.5   \\
%                                          & insert & 96    & 87.5  & 46    & 22.5  & 14    & 81.58 & 74.33 & 51.75 & 27    & 14.5  \\
%                                          & baseline              & 100   & 96.25 & 80    & 65.88 & 55.8  & 63.19 & 68.33 & 67.26 & 63.04 & 58.23 \\ \cmidrule(l){1-12}
% \multirow{4}{*}{lo.}    & both                     & 13.9  & 19.09 & 13.18 & 5.6   & 3.7   & 7.2   & 5     & 3.5   & 3.7   & 2     \\
%                                          & replace     & 73.58 & 37.8  & 16.04 & 7.85  & 3.95  & 20.26 & 7.5   & 5.5   & 3.7   & 2.5   \\
%                                          & insert & 49.48 & 56.44 & 59.09 & 69.61 & 82.24 & 6.92  & 4.62  & 4.95  & 3.42  & 2.5   \\
%                                          & baseline              & 65.24 & 76.86 & 77.64 & 79.4  & 81.64 & 37.26 & 33.28 & 29.77 & 26.76 & 24.38 \\ \cmidrule(l){1-12}
% \multirow{4}{*}{Ll.32} & both                     & 72    & 50.8  & 31.6  & 15.2  & 7.6   & 2.55  & 0.74  & 0.53  & 0.49  & 0.29  \\
%                                          & replace     & 80    & 67.2  & 34.17 & 15.2  & 8.4   & 2.92  & 1.6   & 0.45  & 0.49  & 0.43  \\
%                                          & insert & 66.29 & 45.47 & 45.67 & 52.87 & 57.73 & 3.43  & 0.7   & 0.75  & 1.2   & 1.85  \\
%                                          & baseline              & 66.67 & 65.65 & 65.68 & 65.89 & 65.99 & 27.08 & 23.45 & 20.69 & 18.53 & 16.86 \\ \cmidrule(l){1-12}
% \multirow{4}{*}{yi.}              & both                     & 45.62 & 41.13 & 43.38 & 34.79 & 21.61 & 25.73 & 16.86 & 12.41 & 10.13 & 4.62  \\
%                                          & replace     & 58.88 & 59.09 & 55.81 & 47.78 & 24.74 & 29.72 & 22.63 & 17.92 & 8.02  & 3.07  \\
%                                          & insert & 55.35 & 51.28 & 42.99 & 35.98 & 27.48 & 32    & 30.64 & 21.45 & 12.13 & 16.95 \\
%                                          & baseline              & 71.85 & 68.37 & 65.77 & 62.45 & 56.59 & 30.4  & 30.15 & 29.6  & 29.21 & 28.71 \\ \cmidrule(l){1-12}
% \multirow{4}{*}{vi.}      & both                     & 0     & 0.18  & 0     & 0.17  & 0     & 0     & 0     & 0     & 0     & 0     \\
%                                          & replace     & 0.7   & 0.38  & 0     & 0.17  & 0     & 0     & 0     & 0     & 0     & 0     \\
%                                          & insert & 1.24  & 0.52  & 1.81  & 1.44  & 1.44  & 0     & 0     & 0     & 0     & 0     \\
%                                          & baseline              & 4.29  & 3.64  & 3.09  & 2.72  & 2.47  & 0.91  & 0.78  & 0.68  & 0.61  & 0.54  \\ \cmidrule(l){1-12} 
% \end{tabular}
% }
% \caption{\label{tab:res_factrecall}Results on factrecall tasks. The abbreviations for ch., yi., lo., Ll.32, vi., and Ll.4 represent for Chatglm3-6B-32k, Yi-6B-200k, Longchat-7B-v1.5-32k, Llama-2-7B-32k-Instruct, Vicuna-7B-v1.5-16k, and Llama2-7B-chat-4k, respectively.}
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lc|ccccc|ccccc}
% \hline
% \multirow{2}{*}{model} &
%   \multirow{2}{*}{ablation} &
%   \multicolumn{5}{c|}{factrecall\_en} &
%   \multicolumn{5}{c}{factrecall\_zh} \\
%  &
%    &
%   \multicolumn{1}{l}{$16k$} &
%   \multicolumn{1}{l}{$32k$} &
%   \multicolumn{1}{l}{$64k$} &
%   \multicolumn{1}{l}{$128k$} &
%   \multicolumn{1}{l|}{$256k$} &
%   \multicolumn{1}{l}{$16k$} &
%   \multicolumn{1}{l}{$32k$} &
%   \multicolumn{1}{l}{$64k$} &
%   \multicolumn{1}{l}{$128k$} &
%   \multicolumn{1}{l}{$256k$} \\ \hline
% \multirow{4}{*}{Ll.4}                   & both     & 1.46  & 0.77  & 0.54  & 0.23  & 0.08  & 0     & 0     & 0     & 0     & 0     \\
%                        & replace  & 1.62  & 0.77  & 0.54  & 0.23  & 0.08  & 0     & 0     & 0     & 0     & 0     \\
%                        & insert   & 3.47  & 2.12  & 2.06  & 2.15  & 2.38  & 0     & 0     & 0     & 0     & 0     \\
%                        & baseline & 4.01  & 3.06  & 2.78  & 2.62  & 2.57  & 1.07  & 0.92  & 0.8   & 0.71  & 0.64  \\ \hline
% \multirow{4}{*}{ch.}   & both     & 95.5  & 82    & 44    & 22.25 & 11    & 0     & 2     & 12.5  & 9     & 7     \\
%                        & replace  & 100   & 92.5  & 46.5  & 23.5  & 11.5  & 91.83 & 78    & 41    & 17.17 & 8.5   \\
%                        & insert   & 96    & 87.5  & 46    & 22.5  & 14    & 81.58 & 74.33 & 51.75 & 27    & 14.5  \\
%                        & baseline & 100   & 96.25 & 80    & 65.88 & 55.8  & 63.19 & 68.33 & 67.26 & 63.04 & 58.23 \\ \hline
% \multirow{4}{*}{lo.}   & both     & 13.9  & 19.09 & 13.18 & 5.6   & 3.7   & 7.2   & 5     & 3.5   & 3.7   & 2     \\
%                        & replace  & 73.58 & 37.8  & 16.04 & 7.85  & 3.95  & 20.26 & 7.5   & 5.5   & 3.7   & 2.5   \\
%                        & insert   & 49.48 & 56.44 & 59.09 & 69.61 & 82.24 & 6.92  & 4.62  & 4.95  & 3.42  & 2.5   \\
%                        & baseline & 65.24 & 76.86 & 77.64 & 79.4  & 81.64 & 37.26 & 33.28 & 29.77 & 26.76 & 24.38 \\ \hline
% \multirow{4}{*}{Ll.32} & both     & 72    & 50.8  & 31.6  & 15.2  & 7.6   & 2.55  & 0.74  & 0.53  & 0.49  & 0.29  \\
%                        & replace  & 80    & 67.2  & 34.17 & 15.2  & 8.4   & 2.92  & 1.6   & 0.45  & 0.49  & 0.43  \\
%                        & insert   & 66.29 & 45.47 & 45.67 & 52.87 & 57.73 & 3.43  & 0.7   & 0.75  & 1.2   & 1.85  \\
%                        & baseline & 66.67 & 65.65 & 65.68 & 65.89 & 65.99 & 27.08 & 23.45 & 20.69 & 18.53 & 16.86 \\ \hline
% \multirow{4}{*}{yi.}   & both     & 45.62 & 41.13 & 43.38 & 34.79 & 21.61 & 25.73 & 16.86 & 12.41 & 10.13 & 4.62  \\
%                        & replace  & 58.88 & 59.09 & 55.81 & 47.78 & 24.74 & 29.72 & 22.63 & 17.92 & 8.02  & 3.07  \\
%                        & insert   & 55.35 & 51.28 & 42.99 & 35.98 & 27.48 & 32    & 30.64 & 21.45 & 12.13 & 16.95 \\
%                        & baseline & 71.85 & 68.37 & 65.77 & 62.45 & 56.59 & 30.4  & 30.15 & 29.6  & 29.21 & 28.71 \\ \hline
% \multirow{4}{*}{vi.}   & both     & 0     & 0.18  & 0     & 0.17  & 0     & 0     & 0     & 0     & 0     & 0     \\
%                        & replace  & 0.7   & 0.38  & 0     & 0.17  & 0     & 0     & 0     & 0     & 0     & 0     \\
%                        & insert   & 1.24  & 0.52  & 1.81  & 1.44  & 1.44  & 0     & 0     & 0     & 0     & 0     \\
%                        & baseline & 4.29  & 3.64  & 3.09  & 2.72  & 2.47  & 0.91  & 0.78  & 0.68  & 0.61  & 0.54  \\ \hline
% \end{tabular}%
% }
% \caption{\label{tab:res_factrecall}Results on factrecall tasks. The abbreviations for ch., yi., lo., Ll.32, vi., and Ll.4 represent for Chatglm3-6B-32k, Yi-6B-200k, Longchat-7B-v1.5-32k, Llama-2-7B-32k-Instruct, Vicuna-7B-v1.5-16k, and Llama2-7B-chat-4k, respectively.}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
\multirow{2}{*}{model} & \multirow{2}{*}{ablation}     & \multicolumn{5}{c}{factrecall\_en}                         & \multicolumn{5}{c}{factrecall\_zh}    \\ \cline{3-12} 
 &
   &
  \multicolumn{1}{l}{$16k$} &
  \multicolumn{1}{l}{$32k$} &
  \multicolumn{1}{l}{$64k$} &
  \multicolumn{1}{l}{$128k$} &
  \multicolumn{1}{l}{$256k$} &
  \multicolumn{1}{l}{$16k$} &
  \multicolumn{1}{l}{$32k$} &
  \multicolumn{1}{l}{$64k$} &
  \multicolumn{1}{l}{$128k$} &
  \multicolumn{1}{l}{$256k$} \\ \hline
\multirow{4}{*}{Ll.4}                   & \multicolumn{1}{c|}{both}     & 1.46  & 0.77  & 0.54  & 0.23  & \multicolumn{1}{c|}{0.08}  & 0     & 0     & 0     & 0     & 0     \\
                       & \multicolumn{1}{c|}{replace}  & 1.62  & 0.77  & 0.54  & 0.23  & \multicolumn{1}{c|}{0.08}  & 0     & 0     & 0     & 0     & 0     \\
                       & \multicolumn{1}{c|}{insert}   & 3.47  & 2.12  & 2.06  & 2.15  & \multicolumn{1}{c|}{2.38}  & 0     & 0     & 0     & 0     & 0     \\
                       & \multicolumn{1}{c|}{baseline} & 4.01  & 3.06  & 2.78  & 2.62  & \multicolumn{1}{c|}{2.57}  & 1.07  & 0.92  & 0.8   & 0.71  & 0.64  \\ \hline
\multirow{4}{*}{ch.}   & \multicolumn{1}{c|}{both}     & 95.5  & 82    & 44    & 22.25 & \multicolumn{1}{c|}{11}    & 0     & 2     & 12.5  & 9     & 7     \\
                       & \multicolumn{1}{c|}{replace}  & 100   & 92.5  & 46.5  & 23.5  & \multicolumn{1}{c|}{11.5}  & 91.83 & 78    & 41    & 17.17 & 8.5   \\
                       & \multicolumn{1}{c|}{insert}   & 96    & 87.5  & 46    & 22.5  & \multicolumn{1}{c|}{14}    & 81.58 & 74.33 & 51.75 & 27    & 14.5  \\
                       & \multicolumn{1}{c|}{baseline} & 100   & 96.25 & 80    & 65.88 & \multicolumn{1}{c|}{55.8}  & 63.19 & 68.33 & 67.26 & 63.04 & 58.23 \\ \hline
\multirow{4}{*}{lo.}   & \multicolumn{1}{c|}{both}     & 13.9  & 19.09 & 13.18 & 5.6   & \multicolumn{1}{c|}{3.7}   & 7.2   & 5     & 3.5   & 3.7   & 2     \\
                       & \multicolumn{1}{c|}{replace}  & 73.58 & 37.8  & 16.04 & 7.85  & \multicolumn{1}{c|}{3.95}  & 20.26 & 7.5   & 5.5   & 3.7   & 2.5   \\
                       & \multicolumn{1}{c|}{insert}   & 49.48 & 56.44 & 59.09 & 69.61 & \multicolumn{1}{c|}{82.24} & 6.92  & 4.62  & 4.95  & 3.42  & 2.5   \\
                       & \multicolumn{1}{c|}{baseline} & 65.24 & 76.86 & 77.64 & 79.4  & \multicolumn{1}{c|}{81.64} & 37.26 & 33.28 & 29.77 & 26.76 & 24.38 \\ \hline
\multirow{4}{*}{Ll.32} & \multicolumn{1}{c|}{both}     & 72    & 50.8  & 31.6  & 15.2  & \multicolumn{1}{c|}{7.6}   & 2.55  & 0.74  & 0.53  & 0.49  & 0.29  \\
                       & \multicolumn{1}{c|}{replace}  & 80    & 67.2  & 34.17 & 15.2  & \multicolumn{1}{c|}{8.4}   & 2.92  & 1.6   & 0.45  & 0.49  & 0.43  \\
                       & \multicolumn{1}{c|}{insert}   & 66.29 & 45.47 & 45.67 & 52.87 & \multicolumn{1}{c|}{57.73} & 3.43  & 0.7   & 0.75  & 1.2   & 1.85  \\
                       & \multicolumn{1}{c|}{baseline} & 66.67 & 65.65 & 65.68 & 65.89 & \multicolumn{1}{c|}{65.99} & 27.08 & 23.45 & 20.69 & 18.53 & 16.86 \\ \hline
\multirow{4}{*}{yi.} &
  \multicolumn{1}{c|}{both} &
  45.62 &
  41.13 &
  43.38 &
  34.79 &
  \multicolumn{1}{c|}{21.61} &
  25.73 &
  16.86 &
  12.41 &
  10.13 &
  4.62 \\
                       & \multicolumn{1}{c|}{replace}  & 58.88 & 59.09 & 55.81 & 47.78 & \multicolumn{1}{c|}{24.74} & 29.72 & 22.63 & 17.92 & 8.02  & 3.07  \\
                       & \multicolumn{1}{c|}{insert}   & 55.35 & 51.28 & 42.99 & 35.98 & \multicolumn{1}{c|}{27.48} & 32    & 30.64 & 21.45 & 12.13 & 16.95 \\
                       & \multicolumn{1}{c|}{baseline} & 71.85 & 68.37 & 65.77 & 62.45 & \multicolumn{1}{c|}{56.59} & 30.4  & 30.15 & 29.6  & 29.21 & 28.71 \\ \hline
\multirow{4}{*}{vi.}   & \multicolumn{1}{c|}{both}     & 0     & 0.18  & 0     & 0.17  & \multicolumn{1}{c|}{0}     & 0     & 0     & 0     & 0     & 0     \\
                       & \multicolumn{1}{c|}{replace}  & 0.7   & 0.38  & 0     & 0.17  & \multicolumn{1}{c|}{0}     & 0     & 0     & 0     & 0     & 0     \\
                       & \multicolumn{1}{c|}{insert}   & 1.24  & 0.52  & 1.81  & 1.44  & \multicolumn{1}{c|}{1.44}  & 0     & 0     & 0     & 0     & 0     \\
                       & \multicolumn{1}{c|}{baseline} & 4.29  & 3.64  & 3.09  & 2.72  & \multicolumn{1}{c|}{2.47}  & 0.91  & 0.78  & 0.68  & 0.61  & 0.54  \\ \hline
\end{tabular}%
}
\caption{Results on factrecall tasks. The abbreviations for ch., yi., lo., Ll.32, vi., and Ll.4 represent for ChatGLM3-6B-32k, Yi-6B-200k, LongChat-7B-32k-v1.5, Llama2-7B-32k-Instruct, Vicuna-7B-16k-v1.5, and Llama2-7B-Chat-hf, respectively.}
\label{tab:res_factrecall}
\end{table}

